Wrist Sensor Fusion Enables Robust Gait Quantification Across Walking Scenarios

Quantifying step abundance via single wrist-worn accelerometers is a common approach for encouraging active lifestyle and tracking disease status. Nonetheless, step counting accuracy can be hampered by fluctuations in walking pace or demeanor. Here, we assess whether the use of various sensor fusion techniques, each combining bilateral wrist accelerometer data, may increase step count robustness. By collecting data from 27 healthy subjects, we find that high-level step fusion leads to substantially improved accuracy across diverse walking scenarios. Gait cycle analysis illustrates that wrist devices can recurrently detect steps proximal to toe-off events. Collectively, our study suggests that dual-wrist sensor fusion may enable robust gait quantification in free-living environments.

==> other/table1_unused_version.tex <==
\makeatletter
\def\adl@drawiv#1#2#3{%
        \hskip.5\tabcolsep
        \xleaders#3{#2.5\@tempdimb #1{1}#2.5\@tempdimb}%
                #2\z@ plus1fil minus1fil\relax
        \hskip.5\tabcolsep}
\newcommand{\cdashlinelr}[1]{%
  \noalign{\vskip\aboverulesep
           \global\let\@dashdrawstore\adl@draw
           \global\let\adl@draw\adl@drawiv}
  \cdashline{#1}
  \noalign{\global\let\adl@draw\@dashdrawstore
           \vskip\belowrulesep}}
\makeatother

\begin{table}[hb]
  \caption{Data collection walking tasks. Sample sizes shown after outlier removal.}
  \label{T:setting}
  \centering
  \begin{tabular}{llc}
  \toprule
  \textbf{Category} & \textbf{Walking type} & \textbf{N}\\
  \hhline{---}
  & Slow pace & 25\\
  Unconstrained & Comfortable pace & 26\\
  & Fast pace & 24\\
  \cdashlinelr{1-3}
  & Holding bag in right hand & 27\\
  Arms constrained & Holding cellphone with two hands & 26\\
  & Hands not swinging alongside body & 27\\
  \cdashlinelr{1-3}
  \multirow{2}{*}{Asymmetrical} & Without right shoe & 25\\
  & With imaginary cane in right hand & 23\\
  \hhline{---}
  \textbf{Total} & \textbf{\qquad\qquad\qquad-} & \textbf{203}\\
  \bottomrule
  \end{tabular}
\end{table}

==> other/table2_unused_version.tex <==
\begin{table}[t]
  \caption{Parameter Values. Mean parameter values are shown as determined using 5-fold cross validation with all samples (N=203). The loss function was the root mean square error. Peak detection threshold values are for signal values $\in$ [0, 1], min-max normalized using data from all samples.}
  \centering
  \begin{tabular}{lccccc}
    \toprule
    \multirow{2}{*}{\textbf{Parameter}} & \textbf{Single side} & \multicolumn{2}{c}{\textbf{Low-level fusion}} & \multicolumn{2}{c}{\textbf{High-level fusion}} \\
    \cmidrule(lr){2-2} \cmidrule(lr){3-4} \cmidrule(lr){5-6}
    &  & Sum & Diff & Intersect & Union \\
    \hhline{------}
    \textit{Moving average smoothing}\\
     \hspace{0.5cm}Single sensor window (sec) & 0.03 & 0.18 & 0.02 & 0.02 & 0.40 \\
     \hspace{0.5cm}Fused signal window (sec) & - & 0.08 & 0.02 & - & - \\
         \textit{Peak detection}\\
     \hspace{0.5cm}Min peak amplitude & 0.31 & 0.15 & 0.08 & 0.24 & 0.06 \\
          \hspace{0.5cm}Min window between peaks (sec) & 0.35 & 0.23 & 0.40 & 0.34 & 0.32s \\
     \textit{Event fusion}\\
     \hspace{0.5cm}Max window for peak fusion (sec) & - & - & - & 0.32 & - \\
     \hspace{0.5cm}Min window between peaks (sec) & - & - & - & - & 0.29 \\
    \bottomrule
  \end{tabular}
  \label{T:params}
\end{table}
